An Optimization and Generalization Analysis for Max-Pooling Networks

Max-Pooling operations are a core component of deep learning architectures. In particular, they are part of most convolutional architectures used in machine vision, since pooling is a natural approach to pattern detection problems. However, these architectures are not well understood from a theoretical perspective. For example, we do not understand when they can be globally optimized, and what is the effect of over-parameterization on generalization. Here we perform a theoretical analysis of a convolutional max-pooling architecture, proving that it can be globally optimized, and can generalize well even for highly over-parameterized models. Our analysis focuses on a data generating distribution inspired by pattern detection problem, where a "discriminative" pattern needs to be detected among "spurious" patterns. We empirically validate that CNNs significantly outperform fully connected networks in our setting, as predicted by our theoretical results.

==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}
Understanding the inductive bias of gradient methods for deep learning is an important challenge. In this paper, we study the inductive bias of overparameterized CNNs in a novel setup and provide theoretical and empirical support that SGD exhibits good generalization performance. Our results on MNIST suggest that the PSI phenomenon goes beyond orthogonal patterns.

We use a unique approach of combining novel empirical observations with theoretical guarantees to make headway in a challenging setting of  overparameterized CNNs. We believe that our work can pave the way for studying inductive bias of neural networks in other challenging settings.


%Our PSI inductive bias involves properties of both the training data and the model parameters. In that sense, it is similar to the inductive bias of margin,\footnote{The margin of a sample depends both on the classifier and the training data} but unlike margin, PSI is directly related to the non-linear structure of the model (e.g., the max-pooling operation). 

%Our results raise many exciting questions. Some of these include, proving that SGD converges to a PSI solution for arbitrary training sets, understanding inductive bias for distributions with non-orthogonal patterns and extending the PSI notion to other neural architectures. We leave those for future work.

==> generalization.tex <==
\section{PSI Implies Good Generalization}
\label{sec:generalization}
In the previous section we showed that a general ERM algorithm for the class $\cH$ may need exponentially many training samples to get low test error. Here we show that any algorithm satisfying 
the PSI condition (see Definition \ref{def:psi}) will have low-degree polynomial sample complexity, when patterns in $\cP_s$ are unbiased (i.e., $\expectn{y\mathbbm{1}\{\pp_i \in \xx\}} = 0$ for $\pp_i \in \cP_s$). Specifically, in the following theorem we show that such an algorithm will have zero {\em test} error w.h.p., given only $O(\left|\cP\right|^2\log(\left|\cP\right|))$ training samples. Note that this also implies a sample complexity of $O(d^2\log(d))$ since $\left|\cP\right| \le d$.
%and under the additional assumption that $\cD$ satisfies $\expectn{s_i} = 0$ for all $i \in \cP_m$.

\begin{thm}
\label{thm:du}
Assume that $\cD$ satisfies the conditions in Section \ref{sec:problem_formulation} and $\expectn{y\mathbbm{1}\{\pp_i \in \xx\}} = 0$ for all $\pp_i \in \cP_s$. Let $\cA$ be a learning algorithm which satisfies ($b$,$c$,$\delta$)-PSI with $b,c \ge 1$. Then, if $m > 300b^2c^2\left|\cP\right|^2 \log (\left|\cP\right|)$, with probability at least $1-\delta-\frac{4}{\left|\cP\right|^3}$,\footnote{We note that the $\frac{4}{\left|\cP\right|^3}$ may be improved to an arbitrary $\gamma>0$ if we scale $m$ by $\log{\frac{1}{\gamma}}$.} $\cA(S)$ has $0$ test error.
\end{thm}
We defer the proof to the supplementary but here we sketch the main argument. By the assumption $\expectn{y\mathbbm{1}\{\pp_i \in \xx\}} = 0$ and standard concentration of measure, $\left|s_i\right|$ should be small and therefore the detection ratios should be small by PSI. Then, by the key observation that small detection ratios imply perfect classification (e.g., \eqref{eq:ratio_eq1}), the algorithm achieves zero test error with respect to $\cD$.
\ignore{
\begin{proof}
By the assumption, for $\pp_i \in \cP_s$, $s_i$ is an average of $m$ IID binary variables $y_j \mathbbm{1}\{\pp_i\in \xx_j\}$ with zero expected value.
Thus, by Hoeffding's inequality we have for all $\pp_i \in \cP_s$ that:
\begin{align*}
\prob\left(b\left|s_i\right| \le 4b\sqrt{\frac{\log(d)}{m}}\right) \le \frac{2}{d^4}
\end{align*}
Therefore, by a union bound over all patterns $\pp_i \in \cP_s$ (recall $|\cP|\leq d$), with probability at least $1-\frac{2}{d^3}$, for all $\pp_i \in \cP_s$:
\begin{equation}
\label{eq:bsi_bound}
b\left|s_i\right| \le 4b\sqrt{\frac{\log(d)}{m}} \le \frac{1}{6cd}
\end{equation}
Next we consider $\pp_1$ (the positive pattern), for which $\expectn{s_1}=0.5$ (because it only appears in the positive examples, and the prior over $y$ is $0.5$).
Hoeffding's bound and the definition of $m$ imply that $\left|s_1\right| \ge \frac{1}{3}$ with probability at least  $1 - \frac{1}{d^3}$.\footnote{In fact we can have exponential dependence here, but we use $d^3$ to simplify later expressions.} 

We can now do a union bound over all patterns and PSI condition to obtain that with probability at least $1- \delta-\frac{3}{d^3}$ we have by the PSI property and \eqref{eq:bsi_bound}, for all $\pp_i \in \cP_s$:
\begin{align*}
\label{eq:psi_prop}
\frac{\Miu{+}{i}}{\Miw{+}{1}} \le b\frac{|s_i|}{|s_1|}+\frac{c}{\sqrt{m}} \le
\frac{1}{2cd} + \frac{c}{\sqrt{m}} < \frac{1}{d} \numberthis
\end{align*}
From PSI we have $\frac{\Miu{+}{1}}{\Miw{+}{1}} \le \frac{c}{\sqrt{m}} < \frac{1}{d}$. Therefore, for any positive point $(\xx^+,1)$ \eqref{eq:ratio_eq1} implies:
%
\begin{align*}
    \net\left(\xx^+\right) > \Miw{+}{1}\left(1-\frac{d-1}{d}\right) > 0
\end{align*}

Thus, $\xx^+$ is classified correctly. By the symmetry of the problem and part 2 in Definition \ref{def:psi}, any negative point will be classified correctly as well.
\end{proof}
}

==> inductive_bias.tex <==
\section{Pattern Statistics Inductive Bias}
\label{sec:psi}
The inductive bias of a learning algorithm refers to how the algorithm chooses among all models that fit the data equally well. For example, an SVM algorithm has an inductive bias towards low norm. Understanding the success of deep learning requires understanding the inductive bias of learning algorithms used to learn networks, and in particular SGD \citep{ZhangBHRV16}. 

% To fully understand a learning algorithm, it is desirable to understand properties of this subset of networks, how they depend on the training set and their generalization performance.

In what follows, we define a certain inductive bias of an algorithm in our setting, which we refer to as the Patterns Statistics Inductive Bias (PSI) property. The PSI property states a simple relation between the relative frequency of patterns $s_i$ (see \eqref{eq:psi_def4}) and the detection ratios. We begin by providing the formal definition of PSI, and then provide further intuition. For the definition, we let $\cA$ be any learning algorithm which given a training set $S$ returns a network $\cA(S)$ as in \eqref{eq:network}. 

%We shall show later theoretically that PSI results in good generalization properties, and then show empirically that SGD on neural nets satisfies the PSI property. Taken together these two observations suggest that PSI could serve to explain the practical success of SGD in some cases.


%Intuitively, this makes sense since a pattern that appears in the same frequency in both labels should not be ``interesting'' for the classifier. However, there are models that fit the data that do not satisfy this property, and hence it is interesting to consider it as an inductive bias.


\begin{definition}
\label{def:psi}
We say that a learning algorithm $\cA$ satisfies the Patterns Statistics Inductive Bias condition with constants $b, c, \delta > 0$ (($b$,$c$,$\delta$)-PSI) if the following holds. For any $m \ge 1$, \footnote{We state $m \ge 1$ for simplicity. Alternatively, one can assume $m \ge C$ for a constant $C$.} with probability at least $1-\delta$ over the randomization of $\cA$ and training set $S$ of size $m$, $\cA(S)$ satisfies the following conditions:
% \begin{enumerate}
%     \item For all $i \in \cP_s \cup \cP_+$:
%     \begin{equation}
%     \frac{\Miu{+}{i}}{\Miw{+}{1}} \le b\max\left(-\frac{s_i}{s_1}, 0\right) + \frac{c}{\sqrt{m}}
%     \label{eq:psi_plus}
%     \end{equation}
%     \item For all $i \in \cP_s \cup \cP_-$:
%     \begin{equation}
%     \frac{\Miw{-}{i}}{\Miu{-}{2}} \le b\max\left(-\frac{s_i}{s_2}, 0\right) + \frac{c}{\sqrt{m}}
%     \label{eq:psi_minus}
%     \end{equation}
% \end{enumerate}
% \end{definition}

% \begin{enumerate}
%     \item For all $i \in \cP_s \cup \cP_+$:
\begin{equation}
\forall i \in \cP_s \cup \cP_+: \ \     \frac{\Miu{+}{i}}{\Miw{+}{1}} \le b\max\left(-\frac{s_i}{s_1}, 0\right) + \frac{c}{\sqrt{m}}
\label{eq:psi_plus}
\end{equation}
%\item For all $i \in \cP_s \cup \cP_-$:
\begin{equation}
\forall i \in \cP_s \cup \cP_-: \ \ \frac{\Miw{-}{i}}{\Miu{-}{2}} \le b\max\left(-\frac{s_i}{s_2}, 0\right) + \frac{c}{\sqrt{m}}
\label{eq:psi_minus}
\end{equation}
%\end{enumerate}
\end{definition}

% intuitively captures the properties of network solutions found by gradient descent. In an nutshell, PSI asserts that the statistics of the patterns in the data govern the size of the correlation between a pattern and its detector.

We next provide some \textit{informal} intuition as to why SGD updates may lead to PSI (in \secref{sec:psi_exps} we provide a proof of this for a restricted setting).  

We will consider updates made by gradient descent (full batch SGD). Define $\cW^+_t(i)$ to be the set $\cW^+(i)$ with weight vectors $\wvec{j}_t$ instead of $\wvec{j}$. Similarly, define $\cU^+_t(i)$, $\cW^-_t(i)$ and $\cU^-_t(i)$. Throughout the discussion below, we assume that these sets have roughly the same size.\footnote{This holds with high probability at initialization for a sufficiently large network. Furthermore, in Section \ref{sec:psi_exps}, we show that it holds during training in the case of two training points.} We will show that in certain cases, a high value of $-\frac{s_i}{s_1}$ implies that the detection ratio $\frac{\Miu{+}{i}}{\Miw{+}{1}}$ has a high value. Furthermore, a low value of $-\frac{s_i}{s_1}$ implies a low value of $\frac{\Miu{+}{i}}{\Miw{+}{1}}$. This motivates the bound in the PSI definition. As we will show, this follows since the statistics of the patterns in the training set $s_i$, govern the magnitude of the dot-product between a detector and its detected pattern.

 By our distribution assumption we should have $s_1 \approx \frac{1}{2}$. First assume that $s_i \approx -\frac{1}{2}$ for $\pp_i \in \cP_s$, i.e., $-\frac{s_1}{s_i} \approx 1$. Now lets see what the detection ratio $\frac{\Miu{+}{i}}{\Miw{+}{1}}$ should be by the gradient update. Note that the gradient is a sum of updates, one for each point in the training set. Assume that $j \in \cW^+_t(1)$, i.e., $\wvec{j}$ detects $\pp_1$. Then by the gradient update, the value $\frac{\eta}{m}\pp_1$ is added to $\wvec{j}_{t}$ for \textit{all} positive points that have non-zero hinge loss. The value $-\frac{\eta}{m}\pp_i$ is also added for a few $\pp_i \in \cP_-\cup \cP_s$ and a subset of the negative points ($i$ depends on the specific negative point). In the next iteration, it holds that $j \in \cW^+_{t+1}(1)$ and the updates continue similarly. Overall, we see that $\wvec{j}_{t} \cdot \pp_1$, which is the dot-product between the detector and its detected pattern, increases in each iteration and should be large after a few iterations. Therefore, $\Miw{+}{1}$ should be large. By exactly the same argument, we should expect that for $j \in \cU^+_t(i)$, $\uvec{j}_{t} \cdot \pp_i$ increases in each iteration and now $\Miu{+}{i}$ should be large. Under the assumption that $\left|\cU^+_t(i)\right| \approx \left|\cW^+_t(1)\right|$, we should have $\frac{\Miu{+}{i}}{\Miw{+}{1}} \approx 1$ as well. Therefore, if $-\frac{s_1}{s_i} \approx 1$ then we should expect that $\frac{\Miu{+}{i}}{\Miw{+}{1}} \approx 1$.

On the other hand, if $\pp_i$ appears in roughly an equal number of positive and negative points, i.e., $s_i \approx 0$, then we should expect $\Miu{+}{i}$ to be low. To see this, consider a filter $j \in \cU^+_t(i)$. In this case, positive points that contain $\pp_i$ and with non-zero loss add $-\frac{\eta}{m}\pp_i$ to $\uvec{j}_{t}$, while negative points that contain $\pp_i$ and have non-zero loss add $\frac{\eta}{m}\pp_i$. Thus, $\uvec{j}_{t}\cdot \pp_i$ should not increase signficantly. Therefore, both $\frac{\Miu{+}{i}}{\Miw{+}{1}}$ and $\frac{-s_i}{s_1}$ should be small in this case.

Given the intuition above, one possible conjecture is that the detection ratio $\frac{\Miu{+}{i}}{\Miw{+}{1}}$ is bounded by an affine function of $\max\left(-\frac{s_i}{s_1}, 0\right)$, which leads to the PSI condition in Definition \ref{def:psi}.\footnote{We consider $\max\left(-\frac{s_i}{s_1}, 0\right)$ in the PSI definition because the detection ratios are non-negative.} The bias term in the affine function takes into account that our intuition above is not exact. Finally, we can make a similar argument for $-\frac{s_i}{s_2}$ for motivating \eqref{eq:psi_minus}.

\ignore{
It is reasonable to assume that the bias in the affine function decreases with $m$, because the gradient updates are scaled by $\frac{1}{m}$. Therefore, any additive error in the weights trajectory is scaled by $\frac{1}{m}$. 
}

\ignore{


Given two pattern indices $i_1,i_2$ and any $j \in \cW^+_t(i_1) \cap \cW^-_t(i_2)$ the gradient update is given by:
\begin{equation}
\label{eq:w_gradient}
\wvec{j}_{t+1} = \wvec{j}_{t} + \frac{\eta}{m}\left(\sum_{\xx \in S_{i_1}^+}{\pp_{i_1}\mathbbm{1}_{\nett{t}^k(\xx) < 1}} - \sum_{\xx \in S_{i_2}^-}{\pp_{i_2}\mathbbm{1}_{\nett{t}^k(\xx) < 1}}\right)
\end{equation}
Similarly, for any $j \in \cU^+_t(i_1) \cap \cU^-_t(i_2)$:
\begin{equation}
\label{eq:u_gradient}
\uvec{j}_{t+1} = \uvec{j}_{t} + \frac{\eta}{m}\left(\sum_{\xx \in S_{i_2}^-}{\pp_{i_2}\mathbbm{1}_{\nett{t}^k(\xx) < 1}} - \sum_{\xx \in S_{i_1}^+}{\pp_{i_1}\mathbbm{1}_{\nett{t}^k(\xx) < 1}}\right)
\end{equation}

First assume that $i_1 = 1$ in \eqref{eq:w_gradient}. Since $\pp_1$ appears in all positive points and does not appear in negative points, at iteration $t+1$, $\wvec{j}_{t}\cdot \pp_1$ increases. At iterations $t' > t+1$ it will still hold that $j \in \cW^+_{t'}(1)$, and therefore $\wvec{j}_{t'}\cdot \pp_1$ will continue to increase.
Thus, we should expect that $\Miw{+}{1}$ should be large. Note also that $s_1$ is a large positive number.

Now assume that $i := i_1 = i_2$ in \eqref{eq:u_gradient}, $\pp_i \in P_m$ and $\pp_i$ appears by chance only in negative points in $S$. In this case, $-\frac{s_i}{s_1} \approx 1$. Therefore, by \eqref{eq:u_gradient} we should expect that now $\Miu{+}{i}$ is large and has approximately the same value as $\Miw{+}{1}$ (under our assumption that the sets in \eqref{eq:filters_sets1} and \eqref{eq:filters_sets2} have roughly the same size). Specifically, we see that a large value of $-\frac{s_i}{s_1}$ predicts a large value of $\frac{\Miu{+}{i}}{\Miw{+}{1}}$. 

On the other hand, if $\pp_i$ appears in roughly an equal number of positive and negative points, i.e., $s_i \approx 0$, then we should expect $\Miu{+}{i}$ to be low. To see this, consider the gradient update in \eqref{eq:u_gradient} and consider the corresponding $\uvec{j}_t$ detector for the pattern $\pp_i$. Negative points with the pattern $\pp_i$ increase its norm at iteration $t$, while positive points decrease it. Since there is roughly an equal number of positive points and negative points with pattern $\pp_i$ in $S$, we should expect $\Miu{+}{i}$ to be low. This intuition is not exact because there are the terms $\mathbbm{1}_{\nett{t}^k(\xx) < 1}$, which may be zero for some of the positive or negative points. We note that this is what hinders a theoretical analysis, because $\mathbbm{1}_{\nett{t}^k(\xx) < 1}$ is a random variable which is very hard to analyze. Nevertheless, we still see here that negative points will increase the norm and positive points will decrease the norm. Thus, $\Miu{+}{i}$ should be smaller compared to $\Miw{+}{1}$, which is always increasing. Importantly, we see here that a low value of $-\frac{s_i}{s_1}$ predicts a low value of $\frac{\Miu{+}{i}}{\Miw{+}{1}}$.

We can make a similar argument that $-\frac{s_i}{s_2}$ predicts the value of $\frac{\Miw{-}{i}}{\Miu{-}{2}}$, using the gradient updates in \eqref{eq:w_gradient} and \eqref{eq:u_gradient}.




%The PSI definition below follows this line of thought.

%We see that the PSI definition follows our intuition above. 


%In Section \ref{sec:generalization}, we show that for distributions $\cD$ such that $\expectn{s_i} = 0$ for any $i \in \cP_m$, if $\cA$ satisfies the PSI condition, then its sample complexity to get $0$ test error is $O(b^2c^2d^2\log(d))$. In Section \ref{sec:optimization}, we analyze a setting of two points in the training set and prove that for a sufficiently large network the PSI condition holds for gradient descent. In Section \ref{sec:psi_exps}, we empirically validate that the PSI condition holds for gradient descent and certain distributions $\cD$ with the latter property ($\expectn{s_i} = 0$ for all $i \in \cP_m$). Together these results give firm theoretical and empirical evidence that the sample complexity of gradient descent is $O(d^2\log(d))$. This is despite the result in Section \ref{sec:vc}, which shows existence of networks which overfit and do not satisfy PSI. 
}
%In \secref{sec:generalization} we show that PSI leads to good generalization and in  \secref{sec:psi_exps} we show that PSI empirically holds for our setting. We also prove this for a restricted setting in \secref{sec:optimization}.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}
\newcommand{\commenteps}[1]{}
\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

